Finding Good Proofs for Answers to Conjunctive Queries Mediated by Lightweight Ontologies (Technical Report)

In ontology-mediated query answering, access to incomplete data sources is mediated by a conceptual layer constituted by an ontology. To correctly compute answers to queries, it is necessary to perform complex reasoning over the constraints expressed by the ontology. In the literature, there exists a multitude of techniques incorporating the ontological knowledge into queries. However, few of these approaches were designed for comprehensibility of the query answers. In this article, we try to bridge these two qualities by adapting a proof framework originally applied to axiom entailment for conjunctive query answering. We investigate the data and combined complexity of determining the existence of a proof below a given quality threshold, which can be measured in different ways. By distinguishing various parameters such as the shape of a query, we obtain an overview of the complexity of this problem for the lightweight ontology languages DL-Lite_R and EL, and also have a brief look at temporal query answering.

==> figures/skolemized-proof.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=0.8,
block/.style={
draw,
rounded rectangle,
%minimum width={width("$A \sqsubseteq \exists r.(\exists r.A \sqcap B)$")-5pt}
},
he/.style={rounded corners=10pt,->}]
%extra-begin
\path  (3,3.5) node[block] (x1) {$B(\ex{b})$}
		(9,3.5) node[block] (x2) {$B(y) \to P(y,f(y))$}
		%
		(6,2) node[block] (x3) {$P(\ex{b},f(\ex{b}))$}
		(12,2) node[block] (y0) {$P(y,x)\to S(x,g(x))$}
		(0,2) node[block] (y1) {$P(y,x)\to R(x,y)$}
		%
		(11.5,-0.4) node[block] (y2) {$S(f(\ex{b}),g(f(\ex{b})))$}
		(8.5,0.5) node[block] (y3) {$S(f(\ex{b}),g(f(\ex{b})))$}
		(4,0.5) node[block] (y4) {$R(f(\ex{b}),\ex{b})$}
		(2,-0.4) node[block] (y5) {$R(f(\ex{b}),\ex{b})$}
		(-3.2,-0.4) node[block] (y6){$R(x,y)\to T(y,h(y))$}
		%
        (1,-1.9) node[block] (y7) {$T(\ex{b},h(\ex{b}))$}
        (-1,-2.8) node[block] (y8) {$T(\ex{b},h(\ex{b}))$}
      	%
	     %
	     (4.5,-5) node[block] (z3) {$R(f(\ex{b}),\ex{b}) \,\land\, T(\ex{b},h(\ex{b})) \,\land\, T(\ex{b},h(\ex{b})) \,\land\, R(f(\ex{b}),\ex{b}) \,\land\, S(f(\ex{b}),g(f(\ex{b})))\,\land\, S(f(\ex{b}),g(f(\ex{b})))\,\land\, P(\ex{b},f(\ex{b}))$}
	  (4.5,-6.5) node[block] (z) { $\exists x,x', x'', y, y',z, z'.\, R(x, y) \,\land\, T (y, z) \,\land\, T (y', z) \,\land\, R(x', y') \,\land\,  S(x', z') \,\land\, S(x'', z') \,\land\, P(\ex{b},x'')$};
%\node (x) [block] at (3,3.2) {$B(\ex{b})$};
%\node (y) [draw, rounded rectangle] at (3,2.2) {$P(\ex{b},f(\ex{b}))$};
%\node (z1) [draw, rounded rectangle] at (1,1.2) {$S(f(\ex{b}),g(f(\ex{b})))$};
%\node (z2) [draw, rounded rectangle] at (5,1.2) {$R(f(\ex{b}),\ex{b})$};
%\node (z3) [draw, rounded rectangle] at (5,0.2) {$T(\ex{b},h(\ex{b}))$};
%%extra-end
\draw[he] (x1) -- ($(x1)!0.5!(x2)$) -- (x3);
\draw[he] (x2) -- ($(x1)!0.5!(x2)$) -- (x3);
%
\draw[he] (y0) -- ($(y0)!0.5!(x3)$) -- (y3);
\draw[he] (x3) -- ($(y0)!0.5!(x3)$) -- (y3);
\draw[he] (y0) -- ($(y0)!0.5!(x3)$) -- (y2);
\draw[he] (x3) -- ($(y0)!0.5!(x3)$) -- (y2);
%
\draw[he] (y1) -- ($(y1)!0.5!(x3)$) -- (y4);
\draw[he] (x3) -- ($(y1)!0.5!(x3)$) -- (y4);
\draw[he] (y1) -- ($(y1)!0.5!(x3)$) -- (y5);
\draw[he] (x3) -- ($(y1)!0.5!(x3)$) -- (y5);
%
\draw[he] (y5) -- ($(y5)!0.5!(y6)$) -- (y7);
\draw[he] (y6) -- ($(y5)!0.5!(y6)$) -- (y7);
\draw[he] (y5) -- ($(y5)!0.5!(y6)$) -- (y8);
\draw[he] (y6) -- ($(y5)!0.5!(y6)$) -- (y8);
%%%%
\draw[he] (x3) -- ($(z3)+(0,1)$) --(z3);
\draw[he] (y2)-- ($(z3)+(0,1)$) --(z3);
\draw[he] (y3)-- ($(z3)+(0,1)$) --(z3);
\draw[he] (y4)-- ($(z3)+(0,1)$) --(z3);
\draw[he] (y5)-- ($(z3)+(0,1)$) --(z3);
\draw[he] (y7)-- ($(z3)+(0,1)$) --(z3);
\draw[he] (y8)-- ($(z3)+(0,1)$) --(z3);
\draw[he] (z3) --(z);
%%%%
%\node (d) [draw, rounded rectangle] at (3.2,-1.2) {$R(f(\ex{b}),\ex{b}) \,\land\, T(\ex{b},h(\ex{b})) \,\land\, T(\ex{b},h(\ex{b})) \,\land\, R(f(\ex{b}),\ex{b}) \,\land\, S(f(\ex{b}),g(f(\ex{b})))\,\land\, S(f(\ex{b}),g(f(\ex{b})))\,\land\, P(\ex{b},f(\ex{b}))$};
%\node (e) [draw, rounded rectangle] at (3.2,-2.5) {$\exists x, y, z, y', x', z', x''\, (R(x, y) \,\land\, T (y, z) \,\land\, T (y', z) \,\land\, R(x', y') \,\land\,  S(x', z') \,\land\, S(x'', z') \,\land\, P(\ex{b},x'')$};
%%{$\exists x, z, x', z', x''\, (R(x, \ex{b}) \,\land\, T (\ex{b}, z) \,\land\, T (\ex{b}, z) \,\land\, R(x', \ex{b}) \,\land\,  S(x', z') \,\land\, S(x'', z') \,\land\, P(\ex{b},x'')$};
%%%%
%\draw[he,draw=gray!70] (y)--(d);
%\draw[he,draw=gray!70] (z1)--(d);
%\draw[he,draw=gray!70] (z2)--(d);
%\draw[he,draw=gray!70] (z3)--(d);
%\draw[he] (d)--(e);
\end{tikzpicture}
\caption{A Skolemized proof for Example~\ref{ex}}\label{fig:ex-skolem}
\patrick{I think this can still a bit improved. I would recommend: using
DL notation for TBox axioms, display TBox nodes differently (color or shape),
highlight concluson and premises.}
\end{figure}


==> notes.tex <==
\section{Preliminary Notes}

Basic idea:
\begin{itemize}
\item rewritable DLs:
\item rewriting procedure creates "derivation structure template", where we can cut out non-minimal paths. 
\item to get from this a minimal proof, we need to find that match in the data that would give us the shortest path to the root (the query we are answering). there is an obvious polynomial procedure by just checking, but it looks like there could be a method with lower data complexity
\end{itemize}

Research questions:
\begin{itemize}
\item Data complexity of finding shortest proofs? 

\item The question \enquote{is there a proof of size <k} is not interesting for the data complexity question, since this can be trivially rewritten (just removing the nodes from the derivation template that occur in too long proofs). better would maybe be the question: \enquote{is assertion X involved in the smallest proof?} Now of course this opens up another thing to look at, as we haven't looked at this problem for our previous setting yet.

\item size = tree size = depth or tree-representation, where atoms are first deduced individually and only connected later - that would be a measure where proofs are not paths. 

\item \enquote{Longest intermediate query} on the path or a weighted sum?

\item ABox assertions in the ABox being weighted, for instance using probabilities. Then \enquote{is there a proof of size <k} is not trivial.
\end{itemize}

Easy cases:
\begin{itemize}
 \item For combined complexity, upper bounds follow from our previous results
 \item It seems that for data complexity, for the question ``is there a proof of size<k''  we can often obtain \ACzero upper bounds by using the derivation structure template, and collecting all queries that would give us a proof of size <k, and evaluate them on the data in \ACzero data complexity.
 \begin{itemize}
    \item What happens with ``compute the smallest proof''? We would usually iterate over all values for $k$, but that seems to give us higher data complexity than \ACzero.
 \end{itemize}
\end{itemize}


On derivation structure templates:
\begin{itemize}
    \item The simplest approach would be to compute all rewritings, and add edges
    using entailment checks (or based on how they would be generated, in case we have an
    explicit rewriting procedure)
    \item Already for DL-Lite, this would give us an exponential structure, because there are exponentially many rewritings
    \item Alternative idea would be to just represent atoms in the graph - modulo variable renaming, we have only polynomially many. The last inference step would merge the different atoms together to obtain the final query
    \item Problem with using atoms: how to represent shared variables? We tried a few things ona  meeting on 2022-03-02 and didn't find anything convincing. The problem also comes into place when unification is needed to obtain the rewriting
    \item Possible solution to the problem (suggested by Stefan 22022-03-09): instead of using variables in the pattern, use Skolem constants as they would be introduced in the canonical model construction. Downside: inferences would not be sound in the classical sense anymore. However, as this seems to solve all problems with the variables. We can then think later about how to obtain sound inferences with variables. Another problem: Stefan claimed that
    we only need to consider paths of polyonial length, but then it could still be that we need exponentially many domain elements in total. Since we already have the upper bound for exponential structure, it would be good to get a smaller structure.
    \begin{itemize}
        \item Idea to limit to polynomially many elements: inference graph for each atom in the final query individually, never use the same atom (modulo variable renaming) twice (if an atom would be used twice, we could put the proof for the second occurrence under the proof of the first occurrence). This way, we get polynomially large derivation structures for each atom in the original query, and we can find the shorted path using Dijkstra (the proofs for each atom are always linear for DL-Lite). It looks like this gives us PTime in combined compleity (data complexity is already established as \ACzero).
        \stefan{This assumes that we have only atoms without Skolem terms in the graph, but we have not figured out how to deal with shared variables in this case. If we do consider Skolem terms, then there may be exponentially many possible rewritings for each target atom.}
        \item not clear yet how to deal with unification and shared variables
    \end{itemize}
\end{itemize}


We cannot have trees, even for DL-Lite, because of unification. Data complexity of "optimal size proof" is AC0, combined complexity is in NP (derivation structure is exponential, but we are only looking for polynomially-sized proofs). Is it also NP-hard?

For EL, the derivation structure also contains a "top part" that corresponds to the ABox saturation (i.e., fully instantiated atoms), using the standard entailment rules (e.g., from ELK). Combined complexity is still in NP (same argument as above, the ABox saturation also has polynomial size). For data complexity, the "bottom part" is constant, but in the "top" (polynomial-size) part, we again have to consider sets of atoms, so we have an exponential structure. This would give us only NP even for data complexity ...



\section{Canonical* Model Construction for Explaining Atomic QA}
*H-complete ABox~\cite{DBLP:conf/rweb/KontchakovZ14} (pseudo canonical model that consists of saturated ABox)

In principle, data complexity can be seen as the intensity of the connection between ABox elements and the proof. Therefore, FO-rewriting of atomic queries over LTL ontologies look like \enquote{there is no path which takes the ABox elements and does not produce the atom}. 

For a proof, we may opt for a procedure of bigger data complexity (\eg with a \PTime saturation), but with a clear argumentation. Canonical model can be easily infinite. What if we concentrate only on saturation up to names over the (individual/temporal) domain? 

In other words, even FO-rewriting may be too complicated.
We need either UCQ rewriting with or without ABox saturation.

Given: an ontology and an ABox;
Output: derivation structure.

\paragraph{Atemporal}
\begin{itemize}
\item explain an atomic query (the canonical model construction). For \DLLite -- the derivation structure is finite, no anonymous individuals are needed to derive a fact over a domain element. 
This part is of exp size ($2^{|\Omc|}*|\Amc|$), where $|\Omc|$ bounds the size of the ontology signature and $|\Amc|$ -- the upper bound of the domain size.
For \EL -- we still may need a finite (at most the size of the signature) role chain, then a derivation structure can be bound with $2^{|\Omc|}*|\Amc|*(1+|\Omc|)$.
\end{itemize}

\paragraph{$\Box$ and $\nxt$ in Axioms}
Temporal answer variable ranges over $\mathbb{Z}$:
The canonical model is ultimately periodic. Will it be one derivation structure or a sequence of them? Sequence pros: each DS for a time point is finite; periodicity is a property of the DS sequence. Contras: we need to keep the dependencies between DSs. Best: do not consider the $\mathbb{Z}$ option.

Temporal answer variable ranges over the ABox temporal domain:
The DS is finite. For explanation we still need a phantom zone. Example, ABox $A(a,0)$, TBox $\{A \sqsubseteq \nxt_F B, B \sqsubseteq \Box_P C\}$. The atom $C(a,0)$ holds. The phantom zone can be bounded with an exponent of $\Omc$.

Research questions: small proof?  Results from LPAR can be re-used, since now instead of inference rules we have ``canonical'' model construction. The quotes are because we build a shortened version of it: limited temporal and object domain and restriction to concept and role names.

More ideas: temporal: $\Box$ - polynomially many representative time points outside of ABox (cf. exp many $\Diamond$s in~\cite{DBLP:conf/ruleml/BorgwardtFK19}?) 


%\section{General QA}
%In general, an ontology must normalised. But it does not make a difference for the part we are interested in.
%
%Problem: we do not want to deal with anonymous objects as they are not part of an answer.
%
%Solution: skolemisation or rewriting with tree-witnesses. 
%
%Research question (hardcore): small proof for a query
%Optimize not only rewriting but also the atom derivation.
%\begin{example}
%Consider $q(x)=\exists y. r(x,y) \wedge A(y)$, $\Omc=\{B \sqsubseteq \exists r.C, C\sqsubseteq A\}$ over ABoxes
%$\Amc_1=\{B(a)\}$ and $\Amc_2=\{r(a,b), C(b)\}$.
%
%\begin{tikzpicture}
%\draw[fill=gray!20] (0,0) rectangle (3,0.6) node[anchor=north west] {$\Amc_1$};
%\node at (1.5,0.2) {$B(a)$};
%\node (r2) at (1.5,-0.2) {$B(a)$};
%\node (r1) at (1.5,-1.2) {$\exists y. r(a,y) \wedge C(y)$};
%\node (q) at (1.5,-2.2) {$q(a)$};
%\draw[->] (q) -- (r1);
%\draw[->] (r1) -- (r2); 
%%
%\draw[fill=gray!20] (6,-1) rectangle (9,0.6) node[anchor=north west] {$\Amc_2$};
%\node at (7,0.2) {$r(a,b)$};
%\node (d) at (8,0.2) {$C(b)$};
%\node (s) at (8,-0.8) {$A(b)$};
%\draw[->] (d) -- (s); 
%\node (q2) at (7.5,-1.2) {$q(a)$};
%\end{tikzpicture}
%\end{example}
%
%\begin{lemma}
%For any ABoxes $\Amc_1, \Amc_2$ and $\Amc_3=\Amc_1\cup \Amc_2$, we have
%$$\mathsf{size}(\Omc,q,\Amc_3) \leq \min(\mathsf{size}(\Omc,q,\Amc_1),\mathsf{size}(\Omc,q,\Amc_2)),$$
%where $\mathsf{size}(\Omc,q,\Amc)=\infty$ iff $\Omc,\Amc\not\models q$.
%\end{lemma}
%Trivial.
%
%Query language:  CQ vs rooted. Does it make sense to explain an entailment $\exists x. A(x)$ through $\exists r^- \sqsubseteq A$ and, say,   $B \sqsubseteq \exists t$, $\exists t^- \sqsubseteq \exists s$,  $\exists s^- \sqsubseteq \exists r$ and $B(a)$.
%\section{TCQs: Nodes are annotated with time points}
%Evolution of query
%for each time point - normal proof. Global optimization is about the same proof holds at most other time points
\section{Diamond on the Left}

